Correlation-sensitive magic-state distillation from spin-squeezed neutral atoms

We show that interblock correlations can reverse magic-state distillation even when every input exceeds the threshold for independent states. For the five-to-one Bravyi-Kitaev protocol with independent local Clifford twirls, we express the output in terms of measurable target-axis moments. Fourth-order correlations determine acceptance, while third- and fifth-order correlations determine the output polarization. This relation yields a direct sign test for distillation gain and opposite gains for inputs with identical single-qubit and two-qubit reduced states. We connect this mechanism to neutral-atom resource preparation through finite-range Ising dynamics. Block separation suppresses detrimental interblock coupling, and locally addressed Clifford phases release interaction-generated magic from a spin-squeezed precursor by changing the symmetry selected by code projection. A protocol that retains accepted source outputs achieves positive gain above a source-contrast threshold set by circuit errors and storage dephasing. The same moments specify a finite-sample experimental diagnostic. These results connect the correlation structure of a resource state to its preparation, acceptance, and distillation gain.

==> manuscript_labels.tex <==
% Generated by build.py from the companion document.
\newlabel{fig:circuit}{{1}{2}{}{figure.1}{manuscript.pdf}}
\newlabel{sec:correlation}{{II}{2}{}{section*.4}{manuscript.pdf}}
\newlabel{eq:five-projector}{{1}{2}{}{equation.2.1}{manuscript.pdf}}
\newlabel{eq:general-bloch}{{2}{2}{}{equation.2.2}{manuscript.pdf}}
\newlabel{fig:hierarchical-distillation}{{2}{3}{}{figure.2}{manuscript.pdf}}
\newlabel{eq:sign-mixture}{{3}{3}{}{equation.2.3}{manuscript.pdf}}
\newlabel{eq:moment}{{4}{3}{}{equation.2.4}{manuscript.pdf}}
\newlabel{eq:iid-map}{{5}{3}{}{equation.2.5}{manuscript.pdf}}
\newlabel{fig:moment-sensitivity}{{3}{4}{}{figure.3}{manuscript.pdf}}
\newlabel{eq:ghzt-twirled-comparison}{{6}{4}{}{equation.2.6}{manuscript.pdf}}
\newlabel{sec:clifford}{{III}{4}{}{section*.7}{manuscript.pdf}}
\newlabel{eq:parity-proof}{{7}{4}{}{equation.3.7}{manuscript.pdf}}
\newlabel{sec:finite-range}{{IV}{5}{}{section*.8}{manuscript.pdf}}
\newlabel{eq:array}{{8}{5}{}{equation.4.8}{manuscript.pdf}}
\newlabel{eq:synchronous-yield}{{9}{5}{}{equation.4.9}{manuscript.pdf}}
\newlabel{eq:matched-moment-difference}{{11}{5}{}{equation.4.11}{manuscript.pdf}}
\newlabel{eq:counterexample-conditions}{{12}{5}{}{equation.4.12}{manuscript.pdf}}
\newlabel{fig:array25-moments}{{4}{6}{}{figure.4}{manuscript.pdf}}
\newlabel{sec:readout}{{V}{6}{}{section*.11}{manuscript.pdf}}
\newlabel{eq:readout-main}{{13}{6}{}{equation.5.13}{manuscript.pdf}}
\newlabel{fig:correlation-mechanism}{{5}{7}{}{figure.5}{manuscript.pdf}}
\newlabel{eq:cost-main}{{14}{7}{}{equation.5.14}{manuscript.pdf}}
\newlabel{sec:operating-window}{{VI}{7}{}{section*.12}{manuscript.pdf}}
\newlabel{fig:array}{{6}{8}{}{figure.6}{manuscript.pdf}}
\newlabel{fig:cost}{{7}{8}{}{figure.7}{manuscript.pdf}}
\newlabel{fig:resource-window}{{8}{9}{}{figure.8}{manuscript.pdf}}
\newlabel{fig:diagnostic-flow}{{9}{10}{}{figure.9}{manuscript.pdf}}

